Convolutional Prompting for Broad-Domain Retinal Vessel Segmentation

Previous research on retinal vessel segmentation is targeted at a specific image domain, mostly color fundus photography (CFP). In this paper we make a brave attempt to attack a more challenging task of broad-domain retinal vessel segmentation (BD-RVS), which is to develop a unified model applicable to varied domains including CFP, SLO, UWF, OCTA and FFA. To that end, we propose Dual Convoltuional Prompting (DCP) that learns to extract domain-specific features by localized prompting along both position and channel dimensions. DCP is designed as a plug-in module that can effectively turn a R2AU-Net based vessel segmentation network to a unified model, yet without the need of modifying its network structure. For evaluation we build a broad-domain set using five public domain-specific datasets including ROSSA, FIVES, IOSTAR, PRIME-FP20 and VAMPIRE. In order to benchmark BD-RVS on the broad-domain dataset, we re-purpose a number of existing methods originally developed in other contexts, producing eight baseline methods in total. Extensive experiments show the the proposed method compares favorably against the baselines for BD-RVS.

==> tables/tab_fuse.tex <==
\begin{table}[htb!]
    \caption{\textbf{Performance of different prompt fusion methods}.}
    \label{tab:fuse}
    \renewcommand{\arraystretch}{1.1}
    \centerline{
        \scalebox{0.6}{
            \begin{tabular}{@{}l rrrrrrrr@{}}
               \toprule
                \textbf{Method} 
                %& \textbf{Parameters} & 
                %\textbf{FLOPs} 
                && \textbf{Mean} & \textbf{ROSSA} & \textbf{FIVES} & \textbf{IOSTAR}& \textbf{PRIME-FP20} & \textbf{VAMPIRE} \\
                \midrule
                CP              && 0.7037 & 0.8587 & 0.8928 & 0.8598 & 0.4298 & 0.4776 \\ 
                Multiplication  && 0.6820 & 0.8463 & 0.8776 & 0.8290 & 0.4198 & 0.4371 \\
                Add             && 0.6804 & 0.8427 & 0.8767 & 0.8338 & 0.4085 & 0.4402 \\
                Concat          && 0.6799 & 0.8350 & 0.8837 & 0.8496 & 0.3883 & 0.4431 \\
              \bottomrule
            \end{tabular}
        }
    }
    % \vspace{-0.3cm}
\end{table}
